IndicMT Eval: A Dataset to Meta-Evaluate Machine Translation metrics for Indian Languages

The rapid growth of machine translation (MT) systems has necessitated comprehensive studies to meta-evaluate evaluation metrics being used, which enables a better selection of metrics that best reflect MT quality. Unfortunately, most of the research focuses on high-resource languages, mainly English, the observations for which may not always apply to other languages. Indian languages, having over a billion speakers, are linguistically different from English, and to date, there has not been a systematic study of evaluating MT systems from English into Indian languages. In this paper, we fill this gap by creating an MQM dataset consisting of 7000 fine-grained annotations, spanning 5 Indian languages and 7 MT systems, and use it to establish correlations between annotator scores and scores obtained using existing automatic metrics. Our results show that pre-trained metrics, such as COMET, have the highest correlations with annotator scores. Additionally, we find that the metrics do not adequately capture fluency-based errors in Indian languages, and there is a need to develop metrics focused on Indian languages. We hope that our dataset and analysis will help promote further research in this area.

==> old_tab_corrs_metrics_computed.tex <==
\begin{table*}[]
\scriptsize

\begin{tabular}{lllllllllllllllllll}
                           & \multicolumn{3}{c}{gu}                                                & \multicolumn{3}{c}{hi}                                                & \multicolumn{3}{c}{mr}                                                & \multicolumn{3}{c}{ml}                                                & \multicolumn{3}{c}{ta}                                                & \multicolumn{3}{c}{avg}                                               \\
\multicolumn{1}{c}{Metric} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{K} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{K} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{K} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{K} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{K} & \multicolumn{1}{c}{P} & \multicolumn{1}{c}{S} & \multicolumn{1}{c}{K} \\
BLEU 1                     & 0.364                 & 0.359                 & 0.255                 & 0.266                 & 0.261                 & 0.187                 & 0.228                 & 0.212                 & 0.148                 & 0.393                 & 0.455                 & 0.331                 & 0.316                 & 0.311                 & 0.213                 & 0.314                 & 0.320                 & 0.227                 \\
BLEU 2                     & 0.329                 & 0.346                 & 0.247                 & 0.280                 & 0.269                 & 0.192                 & 0.190                 & 0.193                 & 0.135                 & 0.331                 & 0.404                 & 0.302                 & 0.291                 & 0.291                 & 0.205                 & 0.284                 & 0.301                 & 0.216                 \\
BLEU 3                     & 0.294                 & 0.329                 & 0.234                 & 0.265                 & 0.260                 & 0.186                 & 0.134                 & 0.169                 & 0.119                 & 0.250                 & 0.359                 & 0.271                 & 0.227                 & 0.257                 & 0.182                 & 0.234                 & 0.275                 & 0.198                 \\
BLEU 4                     & 0.235                 & 0.296                 & 0.215                 & 0.245                 & 0.238                 & 0.171                 & 0.091                 & 0.140                 & 0.103                 & 0.180                 & 0.315                 & 0.246                 & 0.171                 & 0.226                 & 0.168                 & 0.184                 & 0.243                 & 0.181                 \\
SacreBLEU                  & 0.293                 & 0.338                 & 0.239                 & 0.255                 & 0.236                 & 0.168                 & 0.164                 & 0.191                 & 0.132                 & 0.274                 & 0.411                 & 0.298                 & 0.244                 & 0.277                 & 0.189                 & 0.246                 & 0.290                 & 0.205                 \\
ROUGE-L                    & 0.350                 & 0.353                 & 0.251                 & 0.295                 & 0.286                 & 0.204                 & 0.206                 & 0.189                 & 0.132                 & 0.376                 & 0.442                 & 0.322                 & 0.308                 & 0.299                 & 0.206                 & 0.307                 & 0.314                 & 0.223                 \\
chrF++                     & 0.408                 & 0.401                 & 0.287                 & 0.299                 & 0.287                 & 0.205                 & 0.260                 & 0.244                 & 0.170                 & 0.411                 & 0.465                 & 0.338                 & 0.361                 & 0.363                 & 0.250                 & 0.348                 & 0.352                 & 0.250                 \\
TER                        & 0.304                 & 0.334                 & 0.237                 & 0.263                 & 0.271                 & 0.196                 & 0.203                 & 0.192                 & 0.135                 & 0.343                 & 0.418                 & 0.307                 & 0.272                 & 0.285                 & 0.199                 & 0.277                 & 0.300                 & 0.215                 \\
EA                         & 0.331                 & 0.257                 & 0.181                 & 0.086                 & 0.093                 & 0.066                 & 0.143                 & 0.079                 & 0.054                 & 0.397                 & 0.413                 & 0.301                 & 0.203                 & 0.220                 & 0.149                 & 0.232                 & 0.212                 & 0.150                 \\
VE                         & 0.380                 & 0.372                 & 0.265                 & 0.274                 & 0.258                 & 0.183                 & 0.234                 & 0.220                 & 0.153                 & 0.412                 & 0.454                 & 0.331                 & 0.337                 & 0.329                 & 0.227                 & 0.327                 & 0.327                 & 0.232                 \\
GM                         & 0.394                 & 0.373                 & 0.266                 & 0.234                 & 0.228                 & 0.162                 & 0.241                 & 0.211                 & 0.147                 & 0.426                 & 0.464                 & 0.338                 & 0.382                 & 0.380                 & 0.264                 & 0.335                 & 0.331                 & 0.235                 \\
mBERT                      & 0.448                 & 0.416                 & 0.297                 & 0.337                 & 0.322                 & 0.231                 & 0.301                 & 0.279                 & 0.194                 & 0.462                 & 0.500                 & 0.367                 & 0.413                 & 0.405                 & 0.281                 & 0.392                 & 0.384                 & 0.274                 \\
distilmBERT                & 0.431                 & 0.406                 & 0.289                 & 0.316                 & 0.308                 & 0.220                 & 0.281                 & 0.260                 & 0.181                 & 0.465                 & 0.505                 & 0.371                 & 0.415                 & 0.399                 & 0.278                 & 0.382                 & 0.376                 & 0.268                 \\
IndicBERT                  & 0.456                 & 0.432                 & 0.308                 & 0.346                 & 0.327                 & 0.235                 & 0.281                 & 0.261                 & 0.182                 & 0.440                 & 0.489                 & 0.357                 & 0.402                 & 0.408                 & 0.282                 & 0.385                 & 0.383                 & 0.273                 \\
MuRIL                      & 0.465                 & 0.449                 & 0.322                 & 0.353                 & 0.339                 & 0.243                 & 0.292                 & 0.264                 & 0.184                 & 0.449                 & 0.504                 & 0.369                 & 0.410                 & 0.419                 & 0.290                 & 0.394                 & 0.395                 & 0.282                                \\
PRISM                      & 0.114                 & 0.035                 & 0.024                 & 0.178                 & 0.176                 & 0.124                 & 0.131                 & 0.122                 & 0.084                 & 0.089                 & 0.091                 & 0.064                 & -0.040                & -0.059                & -0.040                & 0.094                 & 0.073                 & 0.051                 \\
BLEURT-20                  & 0.509                 & 0.520                 & 0.371                 & 0.296                 & 0.410                 & 0.300                 & 0.409                 & 0.407                 & 0.286                 & 0.496                 & 0.526                 & 0.390                 & 0.491                 & 0.532                 & 0.374                 & 0.440                 & 0.479                 & 0.344                 \\
LASER embs                 & 0.094                 & 0.222                 & 0.156                 & 0.135                 & 0.173                 & 0.123                 & 0.159                 & 0.099                 & 0.069                 & 0.357                 & 0.407                 & 0.295                 & 0.126                 & 0.146                 & 0.099                 & 0.174                 & 0.210                 & 0.148                 \\
LabSE embs                 & 0.504                 & 0.448                 & 0.319                 & 0.149                 & 0.258                 & 0.185                 & 0.319                 & 0.294                 & 0.204                 & 0.416                 & 0.466                 & 0.337                 & 0.339                 & 0.412                 & 0.286                 & 0.345                 & 0.376                 & 0.266                \\
COMET-DA                   & 0.557                 & 0.554                 & 0.403                 & 0.581                 & 0.532                 & 0.390                 & 0.426                 & 0.434                 & 0.306                 & 0.531                 & 0.572                 & 0.419                 & 0.529                 & 0.579                 & 0.412                 & 0.525                 & 0.534                 & 0.386  
\end{tabular}
\end{table*}

==> s5_1CorrelationsMQMMetrics.tex <==
\subsection{Metrics Evaluation}
\label{sec:results_1}


%\input{tab_corrs_mqm_metrics}

We compute the pearson and kendall-tau correlations of the MQM formula-based scores and the metric scores on 1400 segments per language. From Table \ref{tab:corr_formula_metrics} 
%we observe an overall ascending order in the performance of word-based metrics such as SacreBLEU, ROUGE-L and TER, followed by embedding-based metrics like  vector extrema, greedy matching, closely followed by the character-level metric, Chrf++.
% We find that the character-level metric, Chrf++, outperforms the embedding-based metrics on languages of Indo-Aryan origin.
%cosine similarity of LabSE embeddings, followed by character-based metric of Chrf++
We also find that computing cosine similarity of the LabSE embeddings of reference and translations yields better correlations than any of the EA,VE and GM approaches using IndicFT embeddings.
The correlations improve further when we use BERTscore applied to different multi-lingual models for getting the embeddings, namely mBERT, distilmBERT, IndicBERT and MuRIL. 

The trained metric PRISM, which has been trained on 39 languages, out of which the only Indian language is Bengali is used since it has been formulated to have zero-shot transferability to other languages. However, we find its performance very poor in all 5 Indian languages in our study, partially owing to the minimal Bengali data used for training.
BLEURT-20, a metric whose backbone RemBERT \cite{rembert} is a 32 layers pre-trained Transformer model (104 languages) finetuned on ratings from the WMT Metrics Shared Task and synthetic data from the WMT corpus has good performance on all languages except Hindi. (We hypothesize that this is due to the relatively richer amount of resources available for Hindi, which in turn leads to several well-performing MT models; and the metric failing at making nuanced/fine-grained distinctions among similar-performing models. This hypothesis is further investigated in section \TODO{xyz}.) 
We find that  COMET-DA is the best-performing metric with good correlations on all the Indian languages considered. 
%We recommend using COMET metric for reliable evaluation of 


%-Also discussion across different parts of the Taxonomy\\
% TODO:
% Vignesh gets NLLB scores for all langs, (simultaneously compute correlations of human vs metric, formula vs metric for NLLB)\\
% - then remove outliers and run correlations on all metrics including nllb -> done(Ananya)\\


\begin{table*}[]
\small
\centering
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\bf Metrics}         & \multicolumn{2}{c}{\bf gu} & \multicolumn{2}{c}{\bf hi} & \multicolumn{2}{c}{\bf mr}  & \multicolumn{2}{c}{\bf ml} & \multicolumn{2}{c}{\bf ta} \\
                & $\rho$    & $\tau$   & $\rho$    & $\tau$   & $\rho$    & $\tau$ & $\rho$    & $\tau$   & $\rho$    & $\tau$   \\
                \midrule
COMET-MQM        & 0.491      & 0.400     & 0.553      & 0.383     & \bf 0.488         & 0.337   & 0.487      & 0.388     & \bf 0.615      & 0.445     \\
Indic-COMET-MQM        & \bf 0.548      & \bf 0.420     & \bf 0.631      & \bf 0.426    & 0.471         & 0.332   & \bf 0.502      & \bf 0.409     & 0.590      & 0.447     \\
\bottomrule
\end{tabular}
\caption{Comparisons between COMET-MQM trained on our MQM data versus the original COMET-MQM dataset. Training on our annotated data clearly helps improve correlations.}
\label{tab:trained_comet_scores}
\end{table*}





==> tab_acc_corr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[[t!]]
\begin{tabular}{lllllllllll}
                                     & \multicolumn{2}{c}{\textbf{gu}}                  & \multicolumn{2}{c}{\textbf{hi}}     & \multicolumn{2}{c}{\textbf{mr}}                               & \multicolumn{2}{c}{\textbf{ml}}                               & \multicolumn{2}{c}{\textbf{ta}}                               \\
\textbf{Metric}                      & \textbf{Pearson} & \textbf{Kendall}              & \textbf{Pearson} & \textbf{Kendall} & \textbf{Pearson}              & \textbf{Kendall}              & \textbf{Pearson}              & \textbf{Kendall}              & \textbf{Pearson}              & \textbf{Kendall}              \\


BLEU 1                               
& 0.397 & 0.268 
& 0.203 & 0.151           
& 0.365 & 0.215 
& 0.515 & 0.388 
& 0.508 & 0.371 \\

BLEU 2                               
& 0.347            & 0.249                         
& 0.212            & 0.155            
& 0.31              & 0.211                         
& 0.43                          & 0.348                         
& 0.413                         & 0.312                         \\
BLEU 3                               
& 0.316            & 0.242                         
& 0.201            & 0.159           
& 0.233                         & 0.203                         
& 0.34                          & 0.313                         
& 0.351                         & 0.275                         \\
BLEU 4                               
& 0.262            & 0.227                         
& 0.2              & 0.156            
& 0.188                         & 0.18                          
& 0.246                         & 0.29                          
& 0.25                          & 0.28                          \\
SacreBLEU                            
& 0.31             & 0.246                         
& 0.201            & 0.156            
& 0.264                         & 0.212                         
& 0.365                         & 0.338                         
& 0.385                         & 0.331                         \\
ROUGE-L                              
& 0.351            & 0.247                         
& 0.223            & 0.154            
& 0.319                         & 0.196                         
& 0.466                         & 0.352                         
& 0.471                         & 0.334                         \\
chrF++                               
& 0.441            & 0.309                         
& 0.219            & 0.164            
& 0.394                         & 0.25                          
& 0.584                         & 0.413                         
& 0.569                         & 0.413                         \\
TER                                  
& -0.319           & -0.232                        
& -0.208           & -0.154           
& -0.355                        & -0.209                        
& -0.439                        & -0.341                        
& -0.421                        & -0.317                        \\
Embedding cosine similarity(IndicFT) 
& 0.297            & 0.19                          
& 0.121            & 0.091            
& 0.352                         & 0.171                         
& 0.551                         & 0.363                         
& 0.512                         & 0.362                         \\
Vector extrema (IndicFT)             
& 0.387            & 0.27                          
& 0.238            & 0.172            
& 0.353                         & 0.214                         
& 0.507                         & 0.356                         
& 0.518                         & 0.376                         \\
Greedy matching  (IndicFT)           
& 0.386            & 0.265                         
& 0.203            & 0.142           
& 0.398                         & 0.219                         
& 0.545                         & 0.383                         
& 0.58                          & 0.42                          \\
mBERT                                
& 0.463            & 0.313                         
& 0.28             & 0.209            
& 0.448                         & 0.278                         
& 0.613                         & 0.434                         
& 0.607 & 0.435                         \\
distilmBERT                          
& 0.449            & 0.309                         
& 0.262            & 0.196            
& 0.4   & 0.249                         
& 0.603                         & 0.42                          
& 0.572                         & 0.409                         \\
IndicBERT                            
& 0.458            & 0.31                          
& 0.272            & 0.184            
& 0.446                         & 0.276                         
& 0.602                         & 0.425                         
& 0.605                         & 0.437                         \\
MuRIL                                
& 0.471            & 0.331                         
& 0.283            & 0.203            
& 0.463                         & 0.283                         
& 0.601                         & 0.436                         
& 0.628                         & 0.461                         \\
COMET-DA                             
& 0.565            & 0.412                         
& 0.44             & 0.313            
& 0.554                         & 0.38                          
& 0.746                         & 0.503                         
& 0.685                         & 0.525                         \\
PRISM                                
& 0.054            & 0.006                         
& 0.086            & 0.078            
& 0.228                         & 0.133                         
& 0.346                         & 0.115                         
& 0.157                         & 0.068                         \\
BLEURT-20                            
& 0.512            & 0.367                         
& 0.151            & 0.194            
& 0.521                         & 0.341                         
& 0.667                         & 0.451                         
& 0.612                         & 0.457                         \\
LASER                                
& 0.103            & 0.171                         
& 0.089            & 0.099            
& 0.364                         & 0.186                         
& 0.547                         & 0.393                         
& 0.246                         & 0.189                         \\
LabSE embs with cosine sim           
& 0.516            & 0.342                        
& 0.074            & 0.116            
& 0.478                         & 0.292                         
& 0.646                         & 0.44                          
& 0.578                         & 0.427                        
\end{tabular}
\end{table*}

==> tab_high_systems.tex <==
\begin{table*}[]
\small
\centering
\begin{tabular}{lllllllllll}
\toprule
            & \multicolumn{2}{c}{\bf gu} & \multicolumn{2}{c}{\bf hi} & \multicolumn{2}{c}{\bf mr} & \multicolumn{2}{c}{\bf ml} & \multicolumn{2}{c}{\bf ta} \\
            
\multirow{-2}{*}{\bf Metrics}        & $\rho$    & $\tau$   & $\rho$    & $\tau$   & $\rho$    & $\tau$   & $\rho$    & $\tau$   & $\rho$    & $\tau$   \\
\midrule
BLEU 1      & 0.225      & 0.151     & 0.191      & 0.136     & 0.208      & 0.135     & 0.259      & 0.211     & 0.213      & 0.141     \\
BLEU 2      & 0.214      & 0.157     & 0.201      & 0.142     & 0.181      & 0.133     & 0.214      & 0.182     & 0.214      & 0.144     \\
BLEU 3      & 0.198      & 0.155     & 0.192      & 0.137     & 0.141      & 0.118     & 0.163      & 0.153     & 0.166      & 0.126     \\
BLEU 4      & 0.162      & 0.139     & 0.173      & 0.126     & 0.114      & 0.11      & 0.114      & 0.133     & 0.123      & 0.111     \\
SacreBLEU   & 0.202      & 0.158     & 0.178      & 0.122     & 0.178      & 0.138     & 0.162      & 0.155     & 0.176      & 0.127     \\
ROUGE-L     & 0.223      & 0.156     & 0.206      & 0.148     & 0.204      & 0.129     & 0.243      & 0.202     & 0.204      & 0.131     \\
CHRF++      & 0.273      & 0.182     & 0.205      & 0.145     & 0.248      & 0.161     & 0.256      & 0.204     & 0.253      & 0.172     \\
TER         & -0.192     & -0.148    & -0.166     & -0.134    & -0.197     & -0.132    & -0.229     & -0.206    & -0.2       & -0.133    \\
\midrule
EA          & 0.208      & 0.081     & 0.044      & 0.021     & 0.098      & 0.024     & 0.183      & 0.143     & 0.089      & 0.076     \\
VE          & 0.288      & 0.188     & 0.185      & 0.126     & 0.198      & 0.128     & 0.252      & 0.202     & 0.241      & 0.161     \\
GM          & 0.282      & 0.171     & 0.159      & 0.108     & 0.212      & 0.128     & 0.256      & 0.199     & 0.269      & 0.19      \\
LASER       & 0.067      & 0.142     & 0.105      & 0.085     & 0.111      & 0.022     & 0.222      & 0.193     & 0.089      & 0.059     \\
LabSE       & 0.372      & 0.218     & 0.119      & 0.129     & 0.27       & 0.163     & 0.337      & 0.243     & 0.232      & 0.218     \\
\midrule
mBERT       & 0.336      & 0.199     & 0.223      & 0.159     & 0.282      & 0.179     & 0.315      & 0.251     & 0.297      & 0.201     \\
distilmBERT & 0.318      & 0.191     & 0.211      & 0.154     & 0.283      & 0.184     & 0.311      & 0.247     & 0.306      & 0.2       \\
IndicBERT   & 0.345      & 0.209     & 0.229      & 0.158     & 0.272      & 0.175     & 0.291      & 0.231     & 0.285      & 0.201     \\
MuRIL       & 0.344      & 0.22      & 0.243      & 0.172     & 0.278      & 0.171     & 0.307      & 0.247     & 0.287      & 0.201     \\
\midrule
PRISM       & 0.148      & 0.015     & 0.138      & 0.096     & 0.123      & 0.074     & 0.065      & 0.044     & -0.109     & -0.081    \\
BLEURT-20   & 0.462      & 0.319     & 0.225      & 0.238     & 0.378      & 0.256     & 0.403      & 0.297     & 0.45       & 0.336     \\
COMET-DA    & 0.525      & 0.349     & 0.448      & 0.3       & 0.404      & 0.27      & 0.452      & 0.326     & 0.49       & 0.376    \\
\bottomrule
\end{tabular}
\caption{Correlations of metric scores with human scores when considering only the top 4 high quality systems, high quality systems are decided using the human scores at the system level. We notice a drop in correlation compared to the values shown in Table~\ref{tab:corr_formula_metrics}}
\label{tab:high_sys_corrs}
\end{table*}

==> tab_hivslo_systems.tex <==

\begin{table*}[t]
\centering
\small
\begin{tabular}{lcccccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{gu}}                  
& \multicolumn{2}{c}{\textbf{hi}}     
& \multicolumn{2}{c}{\textbf{mr}}                               
& \multicolumn{2}{c}{\textbf{ml}}                               
& \multicolumn{2}{c}{\textbf{ta}}                               
\\
\multirow{-2}{*}{\bf Metric}                     
& \textbf{Top} 
& \textbf{Low}              
& \textbf{Top} 
& \textbf{Low}   
& \textbf{Top} 
& \textbf{Low}               
& \textbf{Top} 
& \textbf{Low}                
& \textbf{Top} 
& \textbf{Low}                
\\
\midrule
BLEU 1      & 0.151  & 0.277  & 0.136  & 0.216  & 0.135  & 0.459  & 0.211  & 0.247  & 0.141  & 0.215  \\
BLEU 2      & 0.157  & 0.246  & 0.142  & 0.214  & 0.133  & 0.418  & 0.182  & 0.216  & 0.144  & 0.200  \\
BLEU 3      & 0.155  & 0.225  & 0.137  & 0.203  & 0.118  & 0.388  & 0.153  & 0.165  & 0.126  & 0.166  \\
BLEU 4      & 0.139  & 0.203  & 0.126  & 0.184  & 0.110  & 0.318  & 0.133  & 0.159  & 0.111  & 0.162  \\
SacreBLEU   & 0.158  & 0.243  & 0.122  & 0.177  & 0.138  & 0.438  & 0.155  & 0.246  & 0.127  & 0.191  \\
ROUGE-L     & 0.156  & 0.275  & 0.148  & 0.234  & 0.129  & 0.438  & 0.202  & 0.249  & 0.131  & 0.236  \\
CHRF++      & 0.182  & 0.298  & 0.145  & 0.230  & 0.161  & 0.348  & 0.204  & 0.250  & 0.172  & 0.248  \\
TER         & 0.148 & 0.255 & 0.134 & 0.243 & 0.132 & 0.488 & 0.206 & 0.219 & 0.133 & 0.196 \\

\midrule
EA          & 0.081  & 0.180  & 0.021  & 0.070  & 0.024  & 0.410  & 0.143  & 0.179  & 0.076  & 0.140  \\
VE          & 0.188  & 0.261  & 0.126  & 0.212  & 0.128  & 0.474  & 0.202  & 0.253  & 0.161  & 0.233  \\
GM          & 0.171  & 0.259  & 0.108  & 0.179  & 0.128  & 0.488  & 0.199  & 0.282  & 0.190  & 0.278  \\
LASER embs  & 0.142  & 0.102  & 0.085  & 0.106  & 0.022  & 0.229  & 0.193  & 0.155  & 0.059  & 0.067  \\
LabSE embs  & 0.218  & 0.322  & 0.129  & 0.204  & 0.163  & 0.469  & 0.243  & 0.222  & 0.218  & 0.276  \\
\midrule

mBERT       & 0.199  & 0.294  & 0.159  & 0.291  & 0.179  & 0.509  & 0.251  & 0.313  & 0.201  & 0.304  \\
distilmBERT & 0.191  & 0.295  & 0.154  & 0.271  & 0.184  & 0.479  & 0.247  & 0.329  & 0.200  & 0.308  \\
IndicBERT   & 0.209  & 0.327  & 0.158  & 0.285  & 0.175  & 0.489  & 0.231  & 0.294  & 0.201  & 0.310  \\
MuRIL       & 0.220  & 0.343  & 0.172  & 0.299  & 0.171  & 0.502  & 0.247  & 0.305  & 0.201  & 0.320  \\
\midrule

PRISM       & 0.015  & -0.023 & 0.096  & 0.121  & 0.074  & 0.429  & 0.044  & -0.020 & -0.081 & -0.052 \\
BLEURT-20   & 0.319  & 0.352  & 0.238  & 0.317  & 0.256  & 0.541  & 0.297  & 0.343  & 0.336  & 0.362  \\
COMET-DA    & 0.349  & 0.387  & 0.300  & 0.465  & 0.270  & 0.569  & 0.326  & 0.354  & 0.376  & 0.400 
\\
\bottomrule
\end{tabular}
\caption{Kendall-tau ($\tau$) correlations of the best 4 performing (Top) vs worst 3  performing (Low) systems across the 5 languages. High and Low correspond to the dataset obtained by considering only the best 4 and worst 3 MT systems respectively. We observe that the majority of the metrics show a higher correlation when only the worst systems are considered.}
\label{tab:hi_low_systems}
\end{table*}
